ScaLearn: Simple and Highly Parameter-Efficient Task Transfer by Learning to Scale

Multi-task learning (MTL) has shown considerable practical benefits, particularly when using language models (LMs). While this is commonly achieved by learning $n$ tasks under a joint optimization procedure, some methods, such as AdapterFusion, divide the problem into two stages: (i) task learning, where knowledge specific to a task is encapsulated within sets of parameters (e.g., adapters), and (ii) transfer, where this already learned knowledge is leveraged for a target task. This separation of concerns provides numerous benefits (e.g., promoting reusability). However, current two-stage MTL introduces a substantial number of additional parameters. We address this issue by leveraging the usefulness of linearly scaling the output representations of source adapters for transfer learning. We introduce ScaLearn, a simple and highly parameter-efficient two-stage MTL method that capitalizes on the knowledge of the source tasks by learning a minimal set of scaling parameters that enable effective transfer to a target task. Our experiments on three benchmarks (GLUE, SuperGLUE, and HumSet) and two encoder LMs show that ScaLearn consistently outperforms strong baselines with a small number of transfer parameters (~ $0.35$% of those of AdapterFusion). Remarkably, we observe that ScaLearn maintains its strong abilities even when further reducing parameters, achieving competitive results with only $8$ transfer parameters per target task. Our proposed approach thus demonstrates the power of simple scaling as a promise for more efficient task transfer.

==> 3-analyses.tex <==
%We seek to leverage simple scaling as a novel composition method in two-stage MTL. 

% In this section, we analyze the effects of scaling output representations in transfer learning. 
% We examine these effects by probing the performance of a target task under specific combinations of one or two source tasks. %experiments by (1) scaling the output representations of individual source adapters (single-task probing) and (2) combining two of them, each when training a new task head on target task $t$ (pairwise probing). 
\rev{We seek to leverage simple scaling as a novel composition method in transfer learning. To understand the effect of scaling, we now conduct preliminary experiments in which we scale the output representations of adapters -- in isolation and combining two of them each.}
We use the popular GLUE~\citep{GLUE} and SuperGLUE~\citep{SuperGLUE} benchmarks, utilizing a selection of their tasks (owing to the high number of possible combinations), including entailment, paraphrase detection, sentiment analysis, question answering, and commonsense reasoning tasks. We train a Pfeiffer adapter~\citep{pfeiffer-etal-2021-adapterfusion} on each task using \rev{the encoder PLM} $\text{RoBERTa\textsubscript{BASE}}$~\citep{roberta}. In our probing-like setup~\citep{tenney-etal-2019-bert}, we freeze both the PLM and adapter weights and train a new task head on target task $t$ each time we change the scaling factor. % and Pfeiffer adapters~\citep{pfeiffer-etal-2021-adapterfusion}. %, batch size of $32$, a learning rate of 3e-4, and the Pfeiffer adapter architecture~\citep{pfeiffer-etal-2021-adapterfusion} with a reduction factor of $16$, leading to a bottleneck $\frac{d}{r}$ of size $48$.
Complete descriptions of the datasets, hyperparameters, and training procedure are provided in Section~\ref{sec:setup} and Appendix~\ref{sec:all-hyperparams}. Additional experiments and results on further tasks are provided in Appendix~\ref{sec:all-probing-results}.
% We seek to leverage simple scaling as a novel composition method in 2-stage transfer learning. To understand the effect of scaling, we conduct preliminary experiments in which we scale the output of adapters -- in isolation and combining two of them each.

% Shahed
% Before we formally introduce Scalearn, first we analyze the effect of scaled adapter representations for single task and MTL purposes. For this analysis we conducted two sets of experiments where we used a selection of tasks from GLUE~\citep{GLUE} and SuperGLUE~\citep{SuperGLUE} datasets and trained adapters on an encoder-based PLM $\text{RoBERTa\textsubscript{BASE}}$~\citep{roberta} for each task. Then we either used manually scaled adapter representations and retrained a new task head (Single-task probing) or scaled adapter representations of a source task and add them with manually scaled version of a target task and trained a new task head for the target task (Pariwise probing) and report the accuracy of the model. In the following we discuss the observations from experiments.
% observations

\begin{figure*}[h]
    % \vspace{-2mm}
    \centering
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/st-a_cb_source_0_100.pdf}
        \includegraphics[width=\textwidth]{figures/PPG_cb.pdf}
        \caption{CB}
        \label{fig:fig1.a}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/st-a_copa_source_0_100.pdf}
        \includegraphics[width=\textwidth]{figures/PPG_copa.pdf}
        \caption{COPA}
        \label{fig:fig1.b}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/st-a_mrpc_source_0_100.pdf}
        \includegraphics[width=\textwidth]{figures/PPG_mrpc.pdf}
        \caption{MRPC}
        \label{fig:fig1.c}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/st-a_rte_source_0_100.pdf}
        \includegraphics[width=\textwidth]{figures/PPG_rte.pdf}
        \caption{RTE}
        \label{fig:fig1.d}
    \end{subfigure}
    % \begin{subfigure}{0.18\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/st-a_wsc_source_0_100.pdf}
    %     \caption{WSC}
    %     \label{fig:figa1.a}
    % \end{subfigure}
    
    % \vspace{-3mm}
    \caption{Probing results of 4 target tasks in various transfer learning conditions. (Top) 
    % performance of each target task as we scale the output representation of source adapters.
    Effect of scaling the output representations of adapters by weight $\omega_s$ using different source adapters.
    (Bottom)
    %performance of each target task as we combine independent scaled output representation of MNLI adpter and the respective target task adapter.} 
    Effect of combining independently scaled output representations of two adapters trained on the target task and MNLI, respectively. Each point shows the mean over 5 seeds. Full results are reported in Appendix~\ref{sec:all-probing-results}.}
    \label{fig:fig1}
    % \vspace{-1mm}
\end{figure*}

%\textbf{Single-task probing.} % \label{sec:single-task-probing}
We start by analyzing the performance change of a target task when scaling the output representations of the adapter of \emph{one} given source task. We define $\omega_s$ as the scaling value in the range of $[0,1]$, multiplied by the output representations $\vo^{l}_{s}$ of the source task $s$ in all layers, such that $\vo^{l}_{t} = \omega_{s}\vo^{l}_{s}$. %an adapter by some scalar $\omega$ and its effect on target task performance in encoder-based PLMs. 
% In particular, $\omega$ remains the same for all layers $l$, resulting in $\omega \cdot A^l_S(\bm{x})$. 
%We consider tasks from GLUE~\citep{GLUE} and SuperGLUE~\citep{SuperGLUE} with fewer than 5k samples as target tasks $t$ and all GLUE and SuperGLUE tasks as source tasks.
% Specifically, we take the adapter trained on source task $S$, scale its output representations $A^l_S(\bm{x})$ by $\omega$, and 
%We then train a new task head on target task $t$. The PLM parameters and the adapter parameters $\Theta_t$ remain frozen.
% We show five tasks as source tasks. The remaining tasks with fewer than 5k samples are shown in Appendix~\ref{sec:additional-results}.
% Scaling the output representations $ A^l_\tau(\bm{x})$ of an adapter by $\omega$ reveals several notable characteristics.
% \textbf{Effect of scaling target task representations.} We first consider instances where a new task head is trained using an adapter trained on the \emph{same} task, i.e., $S = T$. Each task demonstrates non-linear changes in performance when scaling $\omega$. First, scaling down $\omega$ significantly decreases performance on most target tasks. Therefore, in the context of adapters, scaling down its representations $A^l_s(\bm{x})$ can be considered as \emph{unlearning} since the task head cannot retrieve the relevant information contained in the adapter parameters. Interestingly, having all the information available, that is, $\omega = 1$, does not necessarily lead to the best performance, as can be observed in task CB (Figure~\ref{fig:fig1.a}) or COPA (Figure~\ref{fig:fig1.b}). In particular, there exist instances where $\omega < 1$ leads to a better performance of the target task than $\omega = 1$, suggesting that \emph{partial learning} of tasks may be beneficial.
% Shortened version:
%When considering instances with $s=t$,  
Figure~\ref{fig:fig1} (Top) shows the probing results on four target tasks (each column), given various scaling weights applied to four source tasks (one of which is the respective target task). The results show that, while increasing the scaling weights generally improves the performance, % reveals that each task demonstrates non-linear changes in performance when scaling $\omega$. Scaling down $\omega$ significantly decreases performance; therefore, scaling down adapter output representations can be considered as \emph{unlearning}. Interestingly, having all the information available, that is, 
the optimal value is not necessarily at $\omega_s=1$. In particular, there exist instances with $0<\omega_s<1$ reaching better performance than $\omega_s = 1$. This suggests that \emph{partial knowledge transfer} of tasks may be more beneficial.
% \textbf{Effect of scaling source task representations.} Next, we consider instances where a new task head is trained on target task $T$ using an adapter trained on source task $S$, with $s \neq t$. Figure~\ref{fig:fig1} (Top) reveals that the performance on target task $T$ is highly dependent on the source adapter used. In fact, given suitable $\omega$, compared to the adapter trained on $T$, the performance on $T$ can be considerably worse, similar, or even better. The latter suggests a strong transfer learning ability for adapters. Of the source tasks, the MNLI-trained adapter performs best. Similarly, MNLI has been shown to exhibit robust task transfer capabilities~\citep{poth-pretrain, intermediate-task-transfer}. Furthermore, there exist other source tasks that are capable of achieving performance comparable to that of the original target task adapter, motivating the \emph{combination} of representations from several task adapters. As in the cases where $c = t$, having all the information contained in $A^l_s(\bm{x})$ ($\omega=1$) can negatively affect performance (considering, for example, $T$ = COPA, $S$ = MNLI), further motivating the usefulness of \textit{partial learning}.
%Considering instances with $s \neq t$, performance on target task $t$ is highly dependent on the source adapter used. 
Notably, and as also reported in previous studies~\citep{poth-pretrain, intermediate-task-transfer}, some source tasks such as MNLI show strong transfer learning abilities. %Of the source tasks, the MNLI-trained adapter performs best. Similarly, MNLI has been shown to exhibit robust task transfer capabilities~\citep{poth-pretrain, intermediate-task-transfer}. 
%Again, transferring all the information contained in $\vo^{l}_{\text{MNLI}}$ ($\omega_\text{MNLI}=1$) might be a sub-optimal for the target task. 


%\textbf{Pairwise probing.} %\label{sec:pairwise-probing}
%Inspired by the usefulness of \emph{partial learning}, 
Next, we go one step further by assessing the scaled \emph{combination} of the output vectors of two adapters. We focus on MNLI as one of the source tasks given its observed benefit in transfer learning, and set the second source adapter (denoted by $s$) to the one corresponding to the target task. We use two scaling parameters $\omega_{\text{MNLI}}$ and $\omega_{s}$ to scale $\vo^{l}_{\text{MNLI}}$ and $\vo^{l}_{s}$, respectively. The resulting output vector is defined as: $\vo^{l}_{t}=\omega_{s}\vo^{l}_{s}+\omega_{\text{MNLI}}\vo^{l}_{\text{MNLI}}$. % We then train a new task head on $t$.
% We consider tasks from GLUE and SuperGLUE with fewer than 10k samples as target tasks.
%For the source task, we use MNLI on the basis of its superior transfer ability.
Figure~\ref{fig:fig1} (Bottom) shows the results for various values of $\omega_{\text{MNLI}}$ and $\omega_{s}$. %  of a selection of target and source tasks when \emph{combining} adapter representations from the MNLI-trained and task adapters. 
Combining the information encapsulated within multiple adapters through scaling can result in improved performance. %compared to only using information encapsulated within a single adapter.
Interestingly, in some cases, the best combination of $\omega_{\text{MNLI}}$ and $\omega_{s}$ does not add up to $1$, i.e., $\omega_{t} + \omega_{s} \neq 1$. 
This finding stands in contrast to the established practice of forcing the scaling coefficients to sum up to 1 (\eg as in \modeladapterfusion, as shown in Eq.~\ref{eq:adapterfusion}).
%However, when multiple vectors are combined into a single vector by scaling their representations, it is commonly assumed that the scaling coefficients add up to 1,
%as exemplified by the softmax function or by taking the mean, both of which are highly common~\citep{dl-relu-softmax}. 
%However, our analyses indicate that this assumption is too restrictive and more of a constraint.
% However, based on our experiments, it seems that this assumption may be too restrictive and more of a constraint.

These initial experiments -- while only covering a simple combination of up to two source tasks -- provide insights into the benefits of scaling representations for transfer learning: (1)~scaling output vectors is an effective method for controlling the (partial or full) activation of the knowledge contained in an adapter module; (2)~an optimal configuration of the scaling parameter will, in many cases, lead to superior results on the target task; (3)~the optimal weights do not necessarily sum up to 1.
%Combined with the competitive performance of other source tasks, 
These observations provide strong motivation for designing a method to \emph{combine} representations from several adapters by scaling their output vectors, presented in the next section.
